Synthetic flow-based cryptomining attack generation through Generative Adversarial Networks

Due to the growing rise of cyber attacks in the Internet, flow-based data sets are crucial to increase the performance of the Machine Learning (ML) components that run in network-based intrusion detection systems (IDS). To overcome the existing network traffic data shortage in attack analysis, recent works propose Generative Adversarial Networks (GANs) for synthetic flow-based network traffic generation. Data privacy is appearing more and more as a strong requirement when processing such network data, which suggests to find solutions where synthetic data can fully replace real data. Because of the ill-convergence of the GAN training, none of the existing solutions can generate high-quality fully synthetic data that can totally substitute real data in the training of IDS ML components. Therefore, they mix real with synthetic data, which acts only as data augmentation components, leading to privacy breaches as real data is used. In sharp contrast, in this work we propose a novel deterministic way to measure the quality of the synthetic data produced by a GAN both with respect to the real data and to its performance when used for ML tasks. As a byproduct, we present a heuristic that uses these metrics for selecting the best performing generator during GAN training, leading to a stopping criterion. An additional heuristic is proposed to select the best performing GANs when different types of synthetic data are to be used in the same ML task. We demonstrate the adequacy of our proposal by generating synthetic cryptomining attack traffic and normal traffic flow-based data using an enhanced version of a Wasserstein GAN. We show that the generated synthetic network traffic can completely replace real data when training a ML-based cryptomining detector, obtaining similar performance and avoiding privacy violations, since real data is not used in the training of the ML-based detector.

==> arXiv copia/figuras/fig-FA-LR.tex <==
\begin{figure*}[!hp]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_400-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_400-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-1}). Training with 400K/4K distribution and one generator chosen uniformly at random}\label{fig:FA_400K-4K}
\end{subfigure}
%


\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/FA-LR_2rnd_0-1_400-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/FA-LR_2rnd_0-1_400-4_Training.png}
\caption{Policy \ref{enum:poli-vainilla-2}). Training with 400K/4K distribution and a mix of two generators is chosen uniformly at random}\label{fig:FA-2_400K-4K}
\end{subfigure}
%

\medskip
\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_4-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-4}). Training with 4K/4K distribution and one generator chosen uniformly at random}\label{fig:FA_4K-4K}
\end{subfigure}
%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using a generator with custom activation functions at the output and policies \ref{enum:poli-vainilla-1}), \ref{enum:poli-vainilla-2}) and \ref{enum:poli-vainilla-4}) (subsection \ref{sec:custom-act-func}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:FA}
\end{minipage}

\end{figure*}

==> arXiv copia/figuras/fig-Mean.tex <==

\begin{figure*}[!tb]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centering
\includegraphics[width=0.49\linewidth]{images/Mean_0-1_400-4_Testing.png} \includegraphics[width=0.49\linewidth]{images/Mean_0-1_400-4_Training.png}
\caption{Unbalanced dataset with the original 400K/4K distribution.}\label{fig:mean_400K-4K}
\end{subfigure}
%

\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Mean_0-1_4-4_Testing.png} \includegraphics[width=0.49\linewidth]{images/Mean_0-1_4-4_Training.png}
\caption{Balanced dataset with 4K/4K distribution.}\label{fig:mean_4K-4K}
\end{subfigure}
%
%
\end{mdframed}

\medskip
%\vspace{1ex}
\begin{minipage}[b]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using a na\"ive mean-based generator with unbalanced and balanced datasets for training (subsection \ref{sec:naive-exp}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented. 
%In (\subref{fig:real_400K-4K}) 400K/4K data distribution was used in tragreen square....
} \label{fig:mean}
\end{minipage}

\end{figure*}



==> arXiv copia/figuras/fig-Real.tex <==

\begin{figure*}[!h]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\includegraphics[width=0.49\linewidth]{images/Real_0-1_400-4_Testing.png} 
\includegraphics[width=0.49\linewidth]{images/Real_0-1_400-4_Training.png}
\caption{F1-score on testing (left) and training (right) using real data for training and testing (400K/4K distribution).}\label{fig:real_400K-4K}
\end{subfigure}
%


\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Real_0-1_4-4_Testing.png} \includegraphics[width=0.49\linewidth]{images/Real_0-1_4-4_Training.png}
\caption{F1-score on testing (left) and training (right) using real data for training and testing (4K/4K distribution).}\label{fig:real_4K-4K}
\end{subfigure}
%


%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using real data  with 400K/4K (\subref{fig:real_400K-4K}) and 4K/4K (\subref{fig:real_4K-4K}) class distributions for training (subsection \ref{sec:experiments-real}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:real}
\end{minipage}
\end{figure*}


==> arXiv copia/figuras/fig-Vainilla-DKJ.tex <==
\begin{figure*}[!h]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_DK_top10_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_DK_top10_1rnd_0-1_4-4_Training.png}}
\caption{Using top $10$ models sorted by $L^1$ distance}
\end{subfigure}
%
\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Vainilla_DJ_top10_1rnd_0-1_4-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/Vainilla_top10_Pos_1rnd_0-1_400-4_Training.png}
\caption{Using top $10$ models sorted by Jaccard index} 
\end{subfigure}

%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{
$F1-score$ on testing (left) and training (right) with sampling elitism using policy \ref{enum:poli-vainilla-1}). Elitism of the top $10$ sorted by statistical coefficients (subsection \ref{sec:elit-metrics}. Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:vainilla-top10-DKJ}
\end{minipage}

\end{figure*}

==> arXiv copia/figuras/fig-Vainilla-Pos.tex <==
\begin{figure*}[!htp]
\begin{mdframed}
\begin{subfigure}[t]{1.\textwidth}
\centerline{
    \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_positivos_0-1_400-4_Testing.png} 
    \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_positivos_0-1_400-4_Training.png}}

\end{subfigure}

\begin{minipage}[t]{1.\textwidth}
\caption{$F1-score$ on testing (left) and training (right) using the discriminator as a quality assurance filter (subsection  \ref{sec:discr-quality-assurance}). Training with 400K/4K distribution. Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.}
\label{fig:vainillaPos_400K-4K}
\end{minipage}
\end{mdframed}
\end{figure*}



==> arXiv copia/figuras/fig-Vainilla-top10.tex <==
\begin{figure*}[!h]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_400-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_400-4_Training.png}}
\caption{Training with 400K/4K distribution. 1 generator chosen uniformly at random}\label{fig:vainilla-top10_400K-4K}
\end{subfigure}
%
\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Vainilla_top10_Pos_1rnd_0-1_400-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/Vainilla_top10_Pos_1rnd_0-1_400-4_Training.png}
\caption{Training with 400K/4K distribution. 1 generator chosen uniformly at random} filtering positive values\label{fig:vainilla-Pos-top10_400K-4K}
\end{subfigure}

\medskip
\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_4-4_Training.png}}
\caption{Training with 4K/4K distribution. 1 generator chosen uniformly at random}\label{fig:vainilla-top10_4K-4K}
\end{subfigure}
%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) with sampling elitism among the top $10$ models in training sorted by $F_1$-score (subsection \ref{subsec:elit_f1}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:vainilla-top10}
\end{minipage}

\end{figure*}

==> arXiv copia/figuras/fig-Vainilla.tex <==
\begin{figure*}[!hp]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_400-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_400-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-1}). Training with 400K/4K distribution and one generator chosen uniformly at random}\label{fig:vainilla_400K-4K}
\end{subfigure}
%
\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Vainilla_2rnd_0-1_400-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/Vainilla_2rnd_0-1_400-4_Training.png}
\caption{Policy \ref{enum:poli-vainilla-2}). Training with 400K/4K distribution and a mix of two generators is chosen uniformly at random}\label{fig:vainilla2_400K-4K}
\end{subfigure}

\medskip
\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_4-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-4}). Training with 4K/4K distribution and one generator chosen uniformly at random}\label{fig:vainilla_4K-4K}
\end{subfigure}
%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using a standard GAN generator and sampling policies \ref{enum:poli-vainilla-1}), \ref{enum:poli-vainilla-2}) and \ref{enum:poli-vainilla-4}) (subsection \ref{sec:results-standard-GAN}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:vainilla}
\end{minipage}

\end{figure*}

==> arXiv copia/figuras/fig_distancias_et0.tex <==


%%%%%%%%%
% et0
%%%%%%%%%


\begin{figure*}[!t]

\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_f1_test.png} 
\caption{$F_1$-score on testing}
\label{fig:vainilla-f1}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_kolmo.png} 
\caption{$L^1$ distance}
\label{fig:vainilla-kolmo}
\end{subfigure}

\medskip

\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_jacc.png} 
\caption{Jaccard index}
\label{fig:vainilla-jac}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_jacc99.png} 
\caption{Jaccard index from percentile 1}
\label{fig:vainilla-jac-1}
\end{subfigure}


\caption{Evolution of $F_1$-score on testing, $L^1$ distance and Jaccard index using GAN generator for label 0. The $x$-axis represents the GAN training epochs.}
\label{fig:distances-vainilla}
\end{figure*}


==> arXiv copia/figuras/fig_distancias_et1.tex <==

%%%%%%%%%
% et1
%%%%%%%%%



\begin{figure*}[!t]


\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et1_f1_test.png} 
\caption{$F_1$-score on testing}\label{fig:vainilla-f1-et1}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et1_kolmo.png} 
\caption{$L^1$ distance}\label{fig:vainilla-kolmo-et1}
\end{subfigure}

\medskip

\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et1_jacc.png} 
\caption{Jaccard index}\label{fig:vainilla-jacc-et1}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et1_jacc99.png} 
\caption{Jaccard index from percentile 1}\label{fig:vainilla-jacc-1-et1}
\end{subfigure}


\caption{Evolution of $F_1$-score on testing, $L^1$ distance and Jaccard index using GAN generator for label 1. The $x$-axis represents GAN training epochs.}
\label{fig:distances-vainilla-et1}
\end{figure*}

==> arXiv copia/figuras/fig_distr_et0-et1.tex <==


%%%%%%%%%
% et0
%%%%%%%%%



\begin{figure*}[!t]
\centering
%et0
\centering
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_1.png} 
\caption{Label 0. Epoch 1}\label{fig:distr-l0-1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_5.png} 
\caption{Label 0. Epoch 5}\label{fig:distr-l0-5}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_200.png} 
\caption{Label 0. Epoch 200}\label{fig:distr-l0-200}
\end{subfigure}
%
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_800.png} 
\caption{Label 0. Epoch 800}\label{fig:distr-l0-800}
\end{subfigure}
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_1500.png} 
\caption{Label 0. Epoch 1000}\label{fig:distr-l0-1500}
\end{subfigure}

\medskip

%et1
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_1.png} 
\caption{Label 1. Epoch 1}\label{fig:distr-l1-1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_5.png} 
\caption{Label 1. Epoch 5}\label{fig:distr-l1-5}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_200.png} 
\caption{Label 1. Epoch 200}\label{fig:distr-l1-200}
\end{subfigure}
%
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_800.png} 
\caption{Label 1. Epoch 800}\label{fig:distr-l1-800}
\end{subfigure}
%
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_1500.png} 
\caption{Label 1. Epoch 1500}\label{fig:distr-l1-1500}
\end{subfigure}
\caption{Comparison of synthetic (blue) and real (red) data distributions using GAN generators for label 0 (\ref{fig:distr-l0-1}, \ref{fig:distr-l0-5}, \ref{fig:distr-l0-200}, \ref{fig:distr-l0-800} and \ref{fig:distr-l0-1500}) and label 1 (\ref{fig:distr-l1-1}, \ref{fig:distr-l1-5}, \ref{fig:distr-l1-200}, \ref{fig:distr-l1-800} and \ref{fig:distr-l1-1500}) in different epochs (1, 5, 200, 800 and 1500). The $4$-dimensional vector has been flattened into by sorting by frequency in ascending order on the $x$-axis.}
\label{fig:comparison-vainilla}
\end{figure*}

==> arXiv copia/figuras/fig_real_distr_et0_et1.tex <==

%%%%%%%%%
% et0
%%%%%%%%%



\begin{figure*}[!t]
\centering
%et0
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f0_real.png} 
\caption{Label 0. Feature 1}\label{fig:distr-real-l0-f1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f1_real.png} 
\caption{Label 0. Feature 2}\label{fig:distr-real-l0-21}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f2_real.png} 
\caption{Label 0. Feature 3}\label{fig:distr-real-l0-f3}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f3_real.png} 
\caption{Label 0. Feature 4}\label{fig:distr-real-l0-f4}
\end{subfigure}
%\hspace*{3em}


\medskip

%et0
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f0_real.png} 
\caption{Label 1. Feature 1}\label{fig:distr-real-l1-f1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f1_real.png} 
\caption{Label 1. Feature 2}\label{fig:distr-real-l1-f2}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f2_real.png} 
\caption{Label 1. Feature 3}\label{fig:distr-real-l1-f3}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f3_real.png} 
\caption{Label 1. Feature 4}\label{fig:distr-real-l1-f4}
\end{subfigure}
%\hspace*{3em}


\caption{Frequency distribution histogram of the 4 variables extracted from normal (Label 0) and cryptomining (label 1) traffic. Label 0 (\ref{fig:distr-l0-1}, \ref{fig:distr-l0-5}, \ref{fig:distr-l0-200}, \ref{fig:distr-l0-800} and \ref{fig:distr-l0-1500}) and label 1 (\ref{fig:distr-l1-1}, \ref{fig:distr-l1-5}, \ref{fig:distr-l1-200}, \ref{fig:distr-l1-800} and \ref{fig:distr-l1-1500}) }
\label{fig:real-data-distribution}
\end{figure*}

==> arXiv copia/tablas/hyperparameters.tex <==
% \usepackage{array}
% \usepackage{graphicx}


\begin{table*}[!t]
\centering
\caption{GAN hyperparameters.}
\label{table:hyperparameters}
\resizebox{0.67\linewidth}{!}{%
\begin{tabular}{>{\hspace{0pt}}m{0.0027\linewidth}>{\hspace{0pt}}m{0.184\linewidth}|>{\hspace{0pt}}m{0.272\linewidth}|>{\hspace{0pt}}m{0.184\linewidth}|}
 & \multicolumn{1}{>{\hspace{0pt}}m{0.204\linewidth}}{} &  & \textbf{Range of values} \\ 
\cline{2-4}
 & \textbf{Generator/discriminator}\par{}\textbf{FCNN architectures} & \textit{\# layers} & {[}2..6] \\ 
\cline{2-4}
 &  & \textit{\# units per layer} & {[}100..10000] \\ 
\cline{2-4}
 & \textbf{Generator} & \textit{Output Activation~} & (linear,custom) \\ 
\cline{2-4}
 &  & Output filtering with discriminator \par{}(\textgreater{}0, percentile) & (True,False)\par{}{[}0..100] \\ 
\cline{3-4}
 &  & \textit{Latent vector }\par{}\textit{with Embedding (categories)} & (True,False)\par{}{[}1..20] \\ 
\cline{3-4}
 &  & latent vector & Fixed 123 \\ 
\cline{3-4}
 &  & noise for latent vector (distr,std) & (normal, uniform)\par{}std=[0.1..100] \\ 
\cline{3-4}
 &  & batch normalization & {[}True..False] \\ 
\cline{3-4}
 &  & regularization: L2, dropout & Fixed values (0,0) \\ 
\cline{3-4}
 &  & learning rate & Default value (0.001) \\ 
\cline{3-4}
 &  & LeakyRelu alpha & Fixed value (0.15) \\ 
\cline{3-4}
 &  & \textit{Percentage of tanh/LeakyRelu }\par{}\textit{in internal units} & {[}0..100] \\ 
\cline{2-4}
 & \textbf{Discriminator}\par{} & \textit{Noise in fakes }\par{}\textit{(distribution,std)} & (normal,uniform)\par{}{[}0..20] \\ 
\cline{2-4}
 &  & \textit{Noise in all examples}\par{}\textit{(distribution,std)} & (normal,uniform)\par{}{[}0..20] \\ 
\cline{3-4}
 &  & \textit{Ratio Label change} & {[}0..20] \\ 
\cline{3-4}
 &  & batch normalization & {[}True..False] \\ 
\cline{3-4}
 &  & regularization: L2, dropout & {[}0..2], [0..30] \\ 
\cline{3-4}
 &  & LeakyRelu alpha & Fixed value (0.2) \\ 
\cline{3-4}
 &  & learning rate & {[}0.0001..0.001] \\ 
\cline{2-4}
 & \textbf{Adaptive~mini-batch} & \textit{generator. ratio fake pass} & Fixed (0.3) \\ 
\cline{2-4}
 &  & \textit{discriminator. ratio TP} & Fixed (0.01) \\ 
\cline{3-4}
 &  & \textit{discriminator. ratio TN} & Fixed (0.01) \\
\cline{3-4}
\end{tabular}
}
\end{table*}

==> arXiv copia/tablas/tabla1.tex <==

%\begin{table}
%\centering
%\caption{Tabla Pepito}
\resizebox{\linewidth}{!}{%
\begin{tabular}{>{\hspace{0pt}}m{0.175\linewidth}|>{\hspace{0pt}}m{0.215\linewidth}|>{\hspace{0pt}}m{0.261\linewidth}|>{\hspace{0pt}}m{0.261\linewidth}|}
\multicolumn{1}{>{\hspace{0pt}}m{0.175\linewidth}}{} &                                                            & Best                                 & Default                               \\ 
\hline
\textbf{400K/4K }\par{}\textbf{1 model}              & \textit{\textbf{threshold}}                                & ~0.8                                 & 0.5                                   \\ 
\hline
                                                     & \textit{\textbf{F1-score}}                                 & 0.927                                & 0.915                                 \\ 
\cline{2-4}
                                                     & \textbf{\textit{Confusion }}\par{}\textbf{\textit{matrix}} & {[}399449 551] \par{}[ 701 ~~~~3687] & {[}399601 399] \par{}[ 983 ~~~~3405]  \\
\cline{2-4}
\end{tabular}
}
%\end{table}

==> arXiv copia/tablas/tabla_Baseline_Medias.tex <==
% \usepackage{array}
% \usepackage{graphicx}

\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Baseline results using a naive mean-based generator for training. }
\label{table:mean}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.732 & 0.664 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 396318 & 3682 \\\hline 1894 & 2493 \end{tabular} & \begin{tabular}{c|c} 390060 & 9940 \\\hline 1416 & 2971 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.601 & 0.583 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377352 & 22648 \\\hline 839 & 3548 \end{tabular} & \begin{tabular}{c|c} 370528 & 29472 \\\hline 537 & 3850 \end{tabular}\\ \hline
\end{tabular}
}
}

\end{table*}


==> arXiv copia/tablas/tabla_FA-Leaky.tex <==
\begin{table}[h!]
%
\parbox{.48\linewidth}{
\caption{Generators using a custom activation function in the output. Results in testing using the best models in training.}
\label{table:FA-Leaky}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.649 & 0.555 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 382755 & 17245 \\\hline  241 & 4146 \end{tabular} & \begin{tabular}{c|c} 357385 & 42615 \\\hline 96 & 4291\end{tabular}\\ \hline\hline
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.622 & 0.559 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377693 & 22307] \\\hline 163 & 4224\end{tabular} & \begin{tabular}{c|c} 358897 & 41103 \\\hline 82 & 4305 \end{tabular}\\ \hline\hline
 
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.532 & 0.467 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 345452 & 54548] \\\hline 21 & 4366\end{tabular} & \begin{tabular}{c|c} 298568 & 101432] \\\hline 0 & 4387\end{tabular}\\ \hline
\end{tabular}
}
}
\end{table}

==> arXiv copia/tablas/tabla_FA-linear-top10.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Results in testing by sampling with elitism among the top $10$ models in training sorted by $F_1$-score. Linear activation function were used in the output layer.}
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top $10$ in $F_1$-score}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} &  0.951 & 0.950 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399800 & 200 \\\hline 608 & 3780 \end{tabular} & \begin{tabular}{c|c} 399832 & 168 \\\hline 658& 3730 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}

==> arXiv copia/tablas/tabla_FA-linear.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Performance metrics of in testing using the best models in training with a synthetic dataset generated by a standard GAN.}
\label{tab:vainilla}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.936 & 0.933 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399926 & 74 \\\hline 927 & 3461 \end{tabular} & \begin{tabular}{c|c} 399962 & 38 \\\hline 998 & 3390 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.927  & 0.915 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399449 & 551 \\\hline 701 & 3687\end{tabular} & \begin{tabular}{c|c} 399601 & 399] \\\hline 983 & 3405 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.878 & 0.835 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399030 & 970 \\\hline 1108 & 3280\end{tabular} & \begin{tabular}{c|c} 396381 & 3619 \\\hline 315 & 4073 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}


==> arXiv copia/tablas/tabla_FA-lnear-top10-KJ-dist.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among the top 10 models in training with $L^1$-distance and Jaccard index.}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 $L^1$-distance}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.869 & 0.858 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399491 & 509 \\\hline 1506 & 2882 \end{tabular} & \begin{tabular}{c|c} 398536 & 1464 \\\hline 1094 & 3294 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 Jaccard index}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.884  & 0.826 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399033 & 967 \\\hline 1031 & 3357\end{tabular} & \begin{tabular}{c|c} 396881 & 3119 \\\hline 720 & 3668 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}

==> arXiv copia/tablas/tabla_FA-top10.tex <==



\begin{table*}[tp]
%
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among top 10 models in training with F1-score }
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\input{tablas/tabla_FA-linear-top10}
}
}
\hfill
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among the top 10 models in training with Kolmogorov distance and Jaccard index}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\input{tablas/tabla_FA-lnear-top10-KJ-dist}
}
}
\end{table*}%



==> arXiv copia/tablas/tabla_FA_filtering.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Performance metrics of in testing using the best models in training after filtering fake samples.}
\label{tab:filtering}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Filtering out fakes}\end{matrix}$}  & \textit{{Threshold}} & 0.6 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.925 & 0.914 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399511 & 489 \\\hline 767 & 3621 \end{tabular} & \begin{tabular}{c|c} 399221 & 779 \\\hline 722 & 3666 \end{tabular}\\ \hline\hline
\end{tabular}
}
}
\end{table*}


==> arXiv copia/tablas/tabla_baseline.tex <==
\begin{table*}[t!]
%
\parbox{.48\linewidth}{
\caption{Baseline results using real data for training.}
\label{table:real}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Real dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.962 & 0.928 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399817 & 183 \\\hline 459 & 3929 \end{tabular} & \begin{tabular}{c|c} 399877 & 123 \\\hline 1008 & 3380 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Real dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.919 & 0.793 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 398602 & 1398 \\\hline 197 & 4191 \end{tabular} & \begin{tabular}{c|c} 394172 & 5828 \\\hline 62 & 4326 \end{tabular}\\ \hline
\end{tabular}
}
}
\hfill
\parbox{.48\linewidth}{
\caption{Baseline results using a naive mean-based generator for training. }
\label{table:mean}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.732 & 0.664 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 396318 & 3682 \\\hline 1894 & 2493 \end{tabular} & \begin{tabular}{c|c} 390060 & 9940 \\\hline 1416 & 2971 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.601 & 0.583 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377352 & 22648 \\\hline 839 & 3548 \end{tabular} & \begin{tabular}{c|c} 370528 & 29472 \\\hline 537 & 3850 \end{tabular}\\ \hline
\end{tabular}
}
}
\medskip
\vspace{3ex}

\parbox{.48\linewidth}{
\caption{Performance of synthetic traffic generated by standard WGANs. Results on testing using the best models on training.}
\label{tab:vainilla}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.936 & 0.933 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399926 & 74 \\\hline 927 & 3461 \end{tabular} & \begin{tabular}{c|c} 399962 & 38 \\\hline 998 & 3390 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.927  & 0.915 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399449 & 551 \\\hline 701 & 3687\end{tabular} & \begin{tabular}{c|c} 399601 & 399 \\\hline 983 & 3405 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.878 & 0.835 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399030 & 970 \\\hline 1108 & 3280\end{tabular} & \begin{tabular}{c|c} 396381 & 3619 \\\hline 315 & 4073 \end{tabular}\\ \hline
\end{tabular}
}
}
\hfill
\parbox{.48\linewidth}{
\caption{Performance of synthetic traffic when generators use  custom activation functions in the output. Results on testing using the best models on training.}
\label{table:FA-Leaky}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.649 & 0.555 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 382755 & 17245 \\\hline  241 & 4146 \end{tabular} & \begin{tabular}{c|c} 357385 & 42615 \\\hline 96 & 4291\end{tabular}\\ \hline\hline
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.622 & 0.559 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377693 & 22307 \\\hline 163 & 4224\end{tabular} & \begin{tabular}{c|c} 358897 & 41103 \\\hline 82 & 4305 \end{tabular}\\ \hline\hline
 
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.532 & 0.467 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 345452 & 54548] \\\hline 21 & 4366\end{tabular} & \begin{tabular}{c|c} 298568 & 101432 \\\hline 0 & 4387\end{tabular}\\ \hline
\end{tabular}
}
}

\medskip
\vspace{3ex}
\parbox{.48\linewidth}{
\caption{Performance of synthetic traffic generated by standard WGANs after filtering fake samples by discriminator. Results on testing using the best models on training.}
\label{tab:filtering}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Filtering out fakes}\end{matrix}$}  & \textit{{Threshold}} & 0.6 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.925 & 0.914 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399511 & 489 \\\hline 767 & 3621 \end{tabular} & \begin{tabular}{c|c} 399221 & 779 \\\hline 722 & 3666 \end{tabular}\\ \hline\hline
\end{tabular}
}
%
\vspace{3ex}
\caption{Performance of synthetic traffic generated by standard WGANs by sampling generators with elitism among the top $10$ models in training sorted by $F_1$-score. Results on testing.}
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top $10$ in $F_1$-score}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} &  0.951 & 0.950 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399800 & 200 \\\hline 608 & 3780 \end{tabular} & \begin{tabular}{c|c} 399832 & 168 \\\hline 658& 3730 \end{tabular}\\ \hline
\end{tabular}
}
}
%
\hfill
\parbox{.48\linewidth}{
\caption{
Performance of synthetic traffic generated by standard WGANs by sampling generators with elitism among the top $10$ models in training sorted by $L^1$-distance and Jaccard index. Results on testing.}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 $L^1$-distance}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.869 & 0.858 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399491 & 509 \\\hline 1506 & 2882 \end{tabular} & \begin{tabular}{c|c} 398536 & 1464 \\\hline 1094 & 3294 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 Jaccard index}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.884  & 0.826 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399033 & 967 \\\hline 1031 & 3357\end{tabular} & \begin{tabular}{c|c} 396881 & 3119 \\\hline 720 & 3668 \end{tabular}\\ \hline
\end{tabular}
}
}

\end{table*}


==> tablas/tabla1.tex <==

%\begin{table}
%\centering
%\caption{Tabla Pepito}
\resizebox{\linewidth}{!}{%
\begin{tabular}{>{\hspace{0pt}}m{0.175\linewidth}|>{\hspace{0pt}}m{0.215\linewidth}|>{\hspace{0pt}}m{0.261\linewidth}|>{\hspace{0pt}}m{0.261\linewidth}|}
\multicolumn{1}{>{\hspace{0pt}}m{0.175\linewidth}}{} &                                                            & Best                                 & Default                               \\ 
\hline
\textbf{400K/4K }\par{}\textbf{1 model}              & \textit{\textbf{threshold}}                                & ~0.8                                 & 0.5                                   \\ 
\hline
                                                     & \textit{\textbf{F1-score}}                                 & 0.927                                & 0.915                                 \\ 
\cline{2-4}
                                                     & \textbf{\textit{Confusion }}\par{}\textbf{\textit{matrix}} & {[}399449 551] \par{}[ 701 ~~~~3687] & {[}399601 399] \par{}[ 983 ~~~~3405]  \\
\cline{2-4}
\end{tabular}
}
%\end{table}

==> tablas/tabla_Baseline_Medias.tex <==
% \usepackage{array}
% \usepackage{graphicx}

\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Baseline results using a naive mean-based generator for training. }
\label{table:mean}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.732 & 0.664 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 396318 & 3682 \\\hline 1894 & 2493 \end{tabular} & \begin{tabular}{c|c} 390060 & 9940 \\\hline 1416 & 2971 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.601 & 0.583 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377352 & 22648 \\\hline 839 & 3548 \end{tabular} & \begin{tabular}{c|c} 370528 & 29472 \\\hline 537 & 3850 \end{tabular}\\ \hline
\end{tabular}
}
}

\end{table*}


==> tablas/tabla_FA-Leaky.tex <==
\begin{table}[h!]
%
\parbox{.48\linewidth}{
\caption{Generators using a custom activation function in the output. Results in testing using the best models in training.}
\label{table:FA-Leaky}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.649 & 0.555 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 382755 & 17245 \\\hline  241 & 4146 \end{tabular} & \begin{tabular}{c|c} 357385 & 42615 \\\hline 96 & 4291\end{tabular}\\ \hline\hline
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.622 & 0.559 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377693 & 22307] \\\hline 163 & 4224\end{tabular} & \begin{tabular}{c|c} 358897 & 41103 \\\hline 82 & 4305 \end{tabular}\\ \hline\hline
 
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.532 & 0.467 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 345452 & 54548] \\\hline 21 & 4366\end{tabular} & \begin{tabular}{c|c} 298568 & 101432] \\\hline 0 & 4387\end{tabular}\\ \hline
\end{tabular}
}
}
\end{table}

==> tablas/tabla_FA-linear-top10.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Results in testing by sampling with elitism among the top $10$ models in training sorted by $F_1$-score. Linear activation function were used in the output layer.}
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top $10$ in $F_1$-score}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} &  0.951 & 0.950 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399800 & 200 \\\hline 608 & 3780 \end{tabular} & \begin{tabular}{c|c} 399832 & 168 \\\hline 658& 3730 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}

==> tablas/tabla_FA-linear.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Performance metrics of in testing using the best models in training with a synthetic dataset generated by a standard GAN.}
\label{tab:vainilla}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.936 & 0.933 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399926 & 74 \\\hline 927 & 3461 \end{tabular} & \begin{tabular}{c|c} 399962 & 38 \\\hline 998 & 3390 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.927  & 0.915 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399449 & 551 \\\hline 701 & 3687\end{tabular} & \begin{tabular}{c|c} 399601 & 399] \\\hline 983 & 3405 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.878 & 0.835 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399030 & 970 \\\hline 1108 & 3280\end{tabular} & \begin{tabular}{c|c} 396381 & 3619 \\\hline 315 & 4073 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}


==> tablas/tabla_FA-lnear-top10-KJ-dist.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among the top 10 models in training with $L^1$-distance and Jaccard index.}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 $L^1$-distance}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.869 & 0.858 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399491 & 509 \\\hline 1506 & 2882 \end{tabular} & \begin{tabular}{c|c} 398536 & 1464 \\\hline 1094 & 3294 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 Jaccard index}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.884  & 0.826 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399033 & 967 \\\hline 1031 & 3357\end{tabular} & \begin{tabular}{c|c} 396881 & 3119 \\\hline 720 & 3668 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}

==> tablas/tabla_FA-top10.tex <==



\begin{table*}[tp]
%
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among top 10 models in training with F1-score }
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\input{tablas/tabla_FA-linear-top10}
}
}
\hfill
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among the top 10 models in training with Kolmogorov distance and Jaccard index}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\input{tablas/tabla_FA-lnear-top10-KJ-dist}
}
}
\end{table*}%



==> tablas/tabla_FA_filtering.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Performance metrics of in testing using the best models in training after filtering fake samples.}
\label{tab:filtering}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Filtering out fakes}\end{matrix}$}  & \textit{{Threshold}} & 0.6 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.925 & 0.914 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399511 & 489 \\\hline 767 & 3621 \end{tabular} & \begin{tabular}{c|c} 399221 & 779 \\\hline 722 & 3666 \end{tabular}\\ \hline\hline
\end{tabular}
}
}
\end{table*}

